To Add Is Machine, To Delete Is Human: Measuring and Mitigating Deletion Avoidance in LLM Code Editing

Large language models increasingly write and repair production code, yet evidence is mounting that their test-passing patches leave codebases harder to maintain. We identify one concrete source: deletion avoidance, the systematic tendency to retain code that an intended edit requires removing. Across the five leading models on the official SWE-bench Verified leaderboard, deletion recall against the developer patch reaches at most 71.7% even on tasks all five solve, and models reach the right file for over 92% of required deletions but cut the exact line in under 52% of cases. Instead, 29.0% of passing patches wrap the targeted code in a guard or fallback, a pattern we call Guard-and-Go. Such patches pass because the original tests rarely check removal: when we retrofit 34 Verified tasks with tests that fail if the targeted code remains, four frontier models spanning closed and open weights fall from 63.2% to 41.9%. Because real repairs mix removal with addition, we curate CanItDelete, a benchmark of 200 tasks mined from real commits whose entire required edit is deletion. Even with the addition work gone, the best model still fails one task in five, and smaller open models fall to 18.0%. We then ablate GPT-5.6 Sol under four cumulative prompts; success moves little until we supply the exact lines, which nearly eliminate incomplete deletion yet raise success only to 80.5% because the model then deletes beyond the spans or adds code instead. Finally, through a pilot study we show one potential fix: teaching deletion during post-training reduces deletion avoidance and improves broader code-editing performance, suggesting the behavior is undertrained rather than beyond reach.

==> Abstract.tex <==
% Write the abstract here.


==> Acknowledgements.tex <==
\begin{acks}
% Add acknowledgments here.
\end{acks}


==> Experiment.tex <==
\section{Study Design}\label{sec:study-design}

% Write the methodology and experimental design here.


==> Implications.tex <==
\section{Discussion}\label{sec:discussion}

% Write the discussion and implications here.


\subsection{When Deletion Becomes Part of the Test Suite}

In RQ1 we have observed that an LLM-generated patch can pass conventional \texttt{FAIL\_TO\_PASS} (F2P) and \texttt{PASS\_TO\_PASS} (P2P) tests while retaining code removed by the official human patch. We therefore examine how benchmark outcomes change when the intended removal is explicitly evaluated through a deletion-focused F2P test.

We begin with 69 SWE-bench Verified tasks in which deletions constitute at least 25\% of the official patch. An AST-aware procedure identifies important code-deletion unit, prioritizing removed conditions, control-flow statements, and complete code blocks while excluding blank lines, comments, docstrings, and trivial structural changes. For tasks whose identified deletion is not covered by the official benchmark tests, we generate a source-level F2P test requiring the targeted code to be absent from its stable enclosing scope. We retain only tests that fail on the base version and pass after applying the official patch, yielding 34 tasks.

Across 136 attempts by four frontier models, 86 (63.2\%) pass without the deletion-focused F2P test, whereas only 57 (41.9\%) pass when it is included, a reduction of 21.3 percentage points. Thus, 29 of the 86 otherwise successful attempts (33.7\%) fail once removal becomes part of the test suite. This reduction occurs for every evaluated model and ranges from 17.7 to 23.5 percentage points.

Benchmark outcomes therefore change materially when deletion becomes part of the evaluation. Because each deletion-focused F2P test is intentionally aligned with the official patch and retained only when the base version fails and the official patch passes, every selected task has a demonstrated solution path through the targeted deletion. Nevertheless, 29 otherwise successful model attempts did not discover a solution satisfying this removal requirement.

Furtehrmore, a small prompt ablation further suggests that mere prompting may be insufficient. For GPT-5.6-Sol, the pass rate decreases from 15/34 without the deletion-motivating prompt to 14/34 with it. In this setting, the prompt did not steer the model toward solutions that were both behaviorally correct and removed enough code to satisfy the deletion-focused F2P test.

These exploratory steps indicate that, when benchmark designers consider removal part of the intended repair, deletion-focused F2P tests can complement conventional F2P and P2P tests. Such evaluations can also expose this capability gap and motivate model developers to train models to perform necessary deletions instead of defaulting to additive workarounds.


==> Prestudy.tex <==
\section{Preliminary Study}\label{sec:preliminary-study}

% Optional: write the preliminary or motivating study here.


==> setup.tex <==
% Shared packages and macros for the paper.
% acmart already loads hyperref, xcolor, amsmath, and booktabs.
\usepackage{xspace}
\usepackage{soul}
\setuldepth{Berlin}
\usepackage{makecell}
\usepackage{balance}
\usepackage{enumitem}
\usepackage{pifont}
\usepackage{float}
\usepackage{csquotes}
\usepackage{ifthen}

\setlength{\textfloatsep}{10pt plus 2pt minus 2pt}
\setlength{\intextsep}{8pt plus 2pt minus 2pt}

\newcommand{\tinyskip}{\vspace{1pt}}
\newcommand{\us}{\_\allowbreak}
\newcommand{\etal}{et~al.~}

% Collaborator comments default to off in tracked source.
% Copy setup.local.tex.example to setup.local.tex to enable visible local review markup.
\newboolean{showcomments}
\setboolean{showcomments}{false}
\InputIfFileExists{setup.local.tex}{}{}

\ifthenelse{\boolean{showcomments}}
{\newcommand{\nbc}[3]{%
  {\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}%
  {\textcolor{#3}{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}%
}}
{\newcommand{\nbc}[3]{}
 \renewcommand{\hl}[1]{#1}}

\newcommand\aadi[1]{\nbc{Aadi}{#1}{blue}}
\newcommand\authorone[1]{\nbc{Author 1}{#1}{red}}
\newcommand\authortwo[1]{\nbc{Author 2}{#1}{orange}}
\newcommand\todo[1]{\nbc{TODO}{#1}{orange}}

\ifthenelse{\boolean{showcomments}}
  {\newcommand\aadistrike[1]{\textcolor{blue}{\st{#1}}}}
  {\newcommand\aadistrike[1]{#1}}

% Reusable result-summary box.
\definecolor{box-blue}{RGB}{25,60,130}
\definecolor{box-gray}{RGB}{248,248,248}
\newtcbtheorem[no counter]{Summary}{\textbf{\small Summary}}{
  enhanced,
  breakable,
  colback=box-gray,
  colframe=box-blue,
  coltitle=white,
  colbacktitle=box-blue,
  boxrule=0.8pt,
  arc=4pt,
  outer arc=4pt,
  top=6pt,
  bottom=2pt,
  left=6pt,
  right=6pt,
  before skip=10pt,
  after skip=10pt,
  attach boxed title to top left={yshift=-2mm,xshift=3mm},
  boxed title style={enhanced,boxrule=0pt,arc=2pt},
  colupper=box-blue
}{summary}

